Regularized Unconstrained Weakly Submodular Maximization

Submodular optimization finds applications in machine learning and data mining. In this paper, we study the problem of maximizing functions of the form $h = f-c$, where $f$ is a monotone, non-negative, weakly submodular set function and $c$ is a modular function. We design a deterministic approximation algorithm that runs with ${{O}}(\frac{n}{\epsilon}\log \frac{n}{\gamma \epsilon})$ oracle calls to function $h$, and outputs a set ${S}$ such that $h({S}) \geq \gamma(1-\epsilon)f(OPT)-c(OPT)-\frac{c(OPT)}{\gamma(1-\epsilon)}\log\frac{f(OPT)}{c(OPT)}$, where $\gamma$ is the submodularity ratio of $f$. Existing algorithms for this problem either admit a worse approximation ratio or have quadratic runtime. We also present an approximation ratio of our algorithm for this problem with an approximate oracle of $f$. We validate our theoretical results through extensive empirical evaluations on real-world applications, including vertex cover and influence diffusion problems for submodular utility function $f$, and Bayesian A-Optimal design for weakly submodular $f$. Our experimental results demonstrate that our algorithms efficiently achieve high-quality solutions.

==> sections/4-theoretical-analysis.tex <==
\subsection{Theoretical Analysis of the Theorems}
\label{sec:theory}





==> sections/7.4-experiments.tex <==
\medskip
\section{Experiments}
\label{sec:experiments} 

The experiments are conducted on a MacBook Pro with M1 Pro chip and 16GB RAM, and all algorithms are implemented in C++. To facilitate a fair comparison among different methods, we have evaluated the computational cost based on the number of function evaluations. 
% Additionally, for profit maximization, we also report the actual running time for fair comparisons to baseline algorithms.
% We have implemented lazy evaluations \cite{minoux2005accelerated} for algorithms with submodular function $f$, for example, ROI and our UP. However, since the algorithms UDG use surrogate submodular functions, lazy evaluations are not applicable because the marginal gains vary unpredictably.
We discuss the applications on profit maximization, vertex cover with costs, and Bayesian A-Optimal design. The latter is specifically for weakly submodular $f$ functions.

\medskip
\textbf{Baseline Algorithms: } 
% As discussed in Section \ref{sec:related}, 
We compare our algorithm \textsc{UP} with \textsc{ROI}~\cite{jin2021unconstrained}, and \textsc{UDG}~\cite{harshaw2019submodular}.
\textsc{ROI} enjoys a tight bound and \textsc{UDG} runs in linear time. Recall that the theoretical bound comparisons are presented in Table~\ref{table:unconstrained}. 
% Note that the theoretical guarantee of ROI in Table~\ref{table:unconstrained} is for a submodular $f$. Thus, when the function $f$ is weakly submodular, as in the Bayesian A-Optimal Design experiment, we use ROI as a heuristic baseline with unknown theoretical guarantees.
The UDG algorithm is randomized and the claimed approximation bounds hold in expectation.
% i.e., $E[f(S) -c(S)] \geq (1-e^{-\gamma})f(OPT) -c(OPT)$. 
Thus, 
% to obtain a high-probability concentration value, one needs to repeat the  algorithm multiple times and consider the median.  In our experiments,
we run the algorithm ten times and report the median objective. As for runtime, we also report the median running time. 


\medskip
\subsection{Profit Maximization}
Information diffusion models \cite{kempe2003maximizing} capture the impact of propagation of information in a network
of connected entities (e.g., social network), where the nodes represent entities (individuals or groups or agencies), and edges
represent the nature of the relationship between entities. The diffusion model is defined using a graph $G=(V,E)$ and a probability function $p(u,v), \forall (u,v)\in E$; 
the probability of an edge denotes the degree of influence of the source node on the destination node connected by the edge.  
A monotone submodular function $f(S) = \mathbb{E}[\mathrm{I}(S)]$ measures the expected number of entities who are influenced by the set of entities in $S$, i.e., if some information
originates at the set $S$, then $\mathrm{I}(S)$ is the number of entities that are likely to receive that information. The function $f$ can be defined following different types of propagation models, such as the independent cascade (IC) model, linear threshold (LT) model~\cite{kempe2003maximizing}, etc. 

Furthermore, it is often the case that there is some cost $c(v)$ associated with each entity $v \in V$ -- this is the cost incurred for including an entity in the seed
set. For instance, a highly influential entity is likely to incur higher costs than others. Following \cite{jin2021unconstrained, tang2018towards}, we use a linear cost function $c:2^V \rightarrow \mathbb{R}^{>0}$ which is proportional to the out-degree of a node $v \in V$.

We define the cost of a single node $v \in V$ as $c(v)$:
\[c(v) = \lambda_1 \cdot d(v)^\lambda_2\] 

where $\lambda_1$ and $\lambda_2$ are positive cost penalty parameters; $d(v)$ is the out-degree of node $v$ and we define $c(v)=1$ if $d(v)=0$ to avoid undefined {\em density} of node $v$. Thus, the modular cost of a set $S \subseteq V$ is $c(S)=\sum_{v\in S}c(v)$. 
Therefore, the {\em profit maximization problem} finds a subset $S$ of $V$ such that:
\[\argmax_{S\subseteq V} ~\mathbb{E}[\mathrm{I}(S)]-c(S)\]

\medskip

\textbf{Profit Maximization Framework Setup}: For fair comparisons, we adapt the profit maximization  framework~\cite{jin2021unconstrained}. For completeness we give a description of their algorithm (Algorithm 2). This algorithm is based on the well-known Random Reachable (RR) approach to speed up the computation of the expected influence value~\cite{borgs2014maximizing,TangXS14,TangSX15,NguyenTD16,HuangWBXL17}. It generates two collections of RR sets with the same size independently; one was given to the algorithm (for example, ROI, UP and UDG) to get a solution set $S$ in line 4; the other collection was unchanged, which was used to verify if the acquired solution set $S$ was a good estimate (line 5 to 7). New collections of RR sets with larger sizes will be re-generated in the next iteration if the solution set $S$ is not a good estimate. So, using Algorithm \ref{alg:pm}, we will iteratively vary the number of RR sets until a satisfied solution set is found. 

In the experiments, we replace function $\mathcal{A}(\cdot)$ with algorithms ROI, UDG, and our UP to find a solution set $S$. In particular, we set $\mathcal{A}(\cdot) =$\textsc{UP}$(\mathcal{R}_1, c, 1, \epsilon)$ for our algorithm \textsc{UP}. Note that  $\mathcal{R}_1$ is given instead of the influence function $f$, but the influence of a set $S$ can be estimated using {\em reverse influence sampling} (RIS) \cite{borgs2014maximizing} technique. The influence of a set $S$ is approximated by $f_{\mathcal{R}}(S)$:

\[f_{\mathcal{R}}(S)=n\frac{Cov_{\mathcal{R}}(S)}{|\mathcal{R}|}\]

where $Cov_{\mathcal{R}}(S)$ is the number of RR sets covered by $S$ and $|\mathcal{R}|$ is the total number of RR sets in $\mathcal{R}$.

Under the framework of Algorithm \ref{alg:pm}, ROI has a approximation guarantee of $f(S)-c(S) \geq (1-\epsilon')f(\OPT)-c(\OPT)-c(\OPT)\log\frac{f(\OPT)}{c(\OPT)}$ \cite{jin2021unconstrained}. When $f$ is submodular in UDG, its guarantee is $\mathbb{E}[f(S)-c(S)] \geq (1-1/e-\epsilon')f(\OPT)-c(\OPT)$~\cite{jin2021unconstrained}. Both guarantees lose $\epsilon'f(\OPT)$ and $\epsilon'$ is the input error threshold in Algorithm \ref{alg:pm}.

\begin{algorithm}[tb]
   \caption{\textsc{PM}($G, f_{\mathcal{R}}, c, \epsilon'$}
   \label{alg:pm}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} graph $G$, spread function with RR sets $f_{\mathcal{R}}$, cost function $c$, error threshold $\epsilon'$
   \STATE {\bfseries Output:} $S$
   \vspace{.05in}
   \STATE $S \gets \emptyset, \theta_0=n, i=1, \delta=1/n$
   \WHILE{$\theta_i \leq (8+2\epsilon')(1+\epsilon_1)n\frac{\log 6/\delta + n \log 2}{\epsilon'^2 \max\{ 1, f_{\mathcal{R}_2}(S) -(1+\epsilon_1)c(S)\}}$}
     \STATE $\mathcal{R}_1, \mathcal{R}_2 \gets$ RR sets with size $\theta_i$ from $G$\\
     \STATE   $S \gets \mathcal{A}(\mathcal{R}_1, c, 1, \epsilon')$
      \STATE  $t\gets (f_{\mathcal{R}_1}(S)-c(S) /(f_{\mathcal{R}_2}(S)-c(S))$
      \STATE  $\epsilon_1 \gets$ larger root of $(\epsilon_1+1)(\epsilon_1+2) / \epsilon_1^2=f_{\mathcal{R}_2}(S) / \ln (6 \cdot i^2 / \delta) \cdot \theta_i / n$
      \STATE  $\epsilon_2 \gets$  larger root of $2( \epsilon_1+1) / \epsilon_2^2= (f_{\mathcal{R}_2}(S^{\circ})-(1+\epsilon_1) c(S^{\circ})) / \log (6 i^2 / \delta) \cdot \theta_i / n $
        \IF{$(t-1) / t+\epsilon_2+\epsilon_1 \leq \epsilon', \epsilon_1+\epsilon_2 \leq \epsilon', \text { and } t, \epsilon_1, \epsilon_2>0$}
         \STATE   Break
        \ENDIF
       \STATE $i++, \theta_i = 2\theta_i$
   \ENDWHILE
\end{algorithmic}
\end{algorithm}



% \begin{algorithm}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \SetKwRepeat{Do}{do}{while}
%     \Input{graph $G$, spread function with RR sets $f_{\mathcal{R}}$, cost function $c$, error threshold $\epsilon'$}
%     \Output{$S$}
%     $S \gets \emptyset, \theta_0=n, i=1, \delta=1/n$\\
%     \While{$\theta_i \leq (8+2\epsilon')(1+\epsilon_1)n\frac{\log 6/\delta + n \log 2}{\epsilon'^2 \max\{ 1, f_{\mathcal{R}_2}(S) -(1+\epsilon_1)c(S)\}}$}{
%         $\mathcal{R}_1, \mathcal{R}_2 \gets$ RR sets with size $\theta_i$ from $G$\\
%         $S \gets \mathcal{A}(\mathcal{R}_1, c, 1, \epsilon')$\\
%         $t\gets (f_{\mathcal{R}_1}(S)-c(S) /(f_{\mathcal{R}_2}(S)-c(S))$\\
%         $\epsilon_1 \gets$ larger root of $(\epsilon_1+1)(\epsilon_1+2) / \epsilon_1^2=f_{\mathcal{R}_2}(S) / \ln (6 \cdot i^2 / \delta) \cdot \theta_i / n$\\
%         $\epsilon_2 \gets$  larger root of $2( \epsilon_1+1) / \epsilon_2^2= (f_{\mathcal{R}_2}(S^{\circ})-(1+\epsilon_1) c(S^{\circ})) / \log (6 i^2 / \delta) \cdot \theta_i / n $\\
%         \If{$(t-1) / t+\epsilon_2+\epsilon_1 \leq \epsilon', \epsilon_1+\epsilon_2 \leq \epsilon', \text { and } t, \epsilon_1, \epsilon_2>0$}{
%             Break
%         }
%         $i++, \theta_i = 2\theta_i$
%     }
%     \caption{\textsc{PM}($G, f_{\mathcal{R}}, c, \epsilon'$) \cite{jin2021unconstrained}}
%     \label{alg:pm}
% \end{algorithm}

\medskip

\textbf{Datasets and Experimental Setup}: We use the standard benchmarks p2p-Gnutella-08 network \cite{leskovec2007graph} and NetHEPT network \cite{chen2009efficient}. p2p-Gnutella-08 \cite{leskovec2007graph} is a collection of sequential snapshots capturing the Gnutella peer-to-peer file-sharing network throughout August 2002. This network consists of $6,301$ nodes and $20,777$ edges, where nodes symbolize hosts within the Gnutella network, while edges denote connections established between these hosts. NetHEPT \cite{chen2009efficient} is an undirected academic collaboration network derived from co-authorships in the ``High Energy Physics - Theory" papers published on arXiv between 1991 and 2003. This network comprises $15,233$ nodes and $62,774$ directed edges, depicting collaborative relationships within the academic domain.

We run the Profit Maximization Algorithms and compare their objective values $(f-c)$ and running time (actual running time in seconds and number of function calls) with various cost penalty choices $\lambda_1$ and $\lambda_2$. We give $\epsilon'=0.2$ and $\delta=1/n$ to Algorithm \ref{alg:pm}. For our algorithm UP, we also test for different error thresholds $\epsilon$: $0.1$, $0.2$ and $0.5$. 

\medskip
\textbf{Effect of $\gamma$}: The results are presented in Figure~\ref{fig:IM-unconstrained-gamma}. For both networks p2p-Gnutella08 and NetHept, we fix $\lambda_1=0.1$, the number of RR sets to be $2^8 \times 10^8$ and vary $\gamma$ from $1.1$ to $1.6$.
In Figure~\ref{fig:IM-unconstrained-gamma}, the two plots on the left showcase the outcome quality derived from both existing algorithms and our proposed algorithm across different $\lambda_2$ (cost parameter) values. These plots demonstrate that our results (blue-diamond line: our UP($\epsilon=0.1$), cyan-circle line: our UP($\epsilon=0.2$ and teal-triangle line: our UP($\epsilon=0.5$) are close to the best-approximation algorithm ROI greedy algorithm (black-dot line) and exhibit a 15\% improvement over UDG (teal-diamond line). Regarding computational efficiency, our algorithm matches the efficiency of the UDG algorithm in terms of the number of function calls and is 6.8 times quicker than ROI. Moreover, our algorithms showcase efficiency akin to ROI concerning actual running time (as denoted by the blue bars). 

\smallskip
\textbf{Effect of $\lambda_2$}: For p2p-Gnutella08 and NetHept, we maintain fixed values of $\lambda_2=1.2$ and $\lambda_2=1.0$, respectively. We generate a total of $2^8 \times 10^8$ RR sets, altering $\lambda_2$ across values ranging from $[0.1, 0.2, 0.3, 0.4, 0.5, 0.6]$. The corresponding outcomes are depicted in Figure \ref{fig:IM-unconstrained-lambda}. Notably, UP demonstrates superior performance compared to UDG, exhibiting a discernible gap between the two methods. When the error thresholds are set at $\epsilon=0.1$ and $\epsilon=0.2$, the quality of results closely aligns with those obtained using ROI. For the p2p-Gnutella-08 network, our algorithm with $\epsilon=0.5$ performs slightly worse than ROI. Nevertheless, it still exhibits a noticeable improvement (approximately 14.8\%) over UDG and maintains a near-linear time complexity (see the third sub-plot of Figure~\ref{fig:IM-unconstrained-lambda} where the y-axis is regularized by logarithm).

% \textbf{Effect of RR sets:} We explore the impact of varying the number of RR sets from $2 \times 10^5$ to $2^9 \times 10^5$. Concurrently, we calculate the actual running time instead of function calls while maintaining fixed cost penalties. Specifically, for p2p-Gnutella08 and NetHept, we set $\lambda=0.1, \gamma=1.2$ and $\lambda=0.2, \gamma=1.0$, respectively. Within the Profit Maximization Algorithm framework, the running time primarily hinges on the RR sets' size generated in Algorithm \ref{alg:pm} and the selection procedure $\mathcal{A(\cdot)}$ outlined in line 4. Figures \ref{fig:IM-unconstrained-rr-obj} and \ref{fig:IM-unconstrained-rr-time-s} depict that the ROI algorithm exhibits the slowest running time due to its quadratic solution set selection process. Conversely, our UP algorithm and UDG swiftly achieve a solution. Notably, our algorithm outperforms UDG by approximately 16\%.

\begin{figure}[t]
\centering
\subfigure[$\lambda_1$ vs $f-c$ with $\lambda_2=1.2$]{
\centering
\includegraphics[width=0.22\textwidth]{figures/p2p-2.pdf}
}
\subfigure[$\lambda_2$ vs $f-c$ with $\lambda_1=0.1$]{
\centering
\includegraphics[width=0.22\textwidth]{figures/p2p-1.pdf}
% \caption{}
}
\label{fig:p2p}
\caption{Comparisons on p2p-Gnutella31 network with Influence Maximization.}
\end{figure}


\begin{figure}[t]
\centering
\subfigure[$\lambda_1$ vs $f-c$ with $\lambda_2=1.0$]{
\centering
\includegraphics[width=0.22\textwidth]{figures/nethept-2.pdf}
}
\subfigure[$\lambda_2$ vs $f-c$ with $\lambda_1=0.1$]{
\centering
\includegraphics[width=0.22\textwidth]{figures/nethept-1.pdf}
% \caption{}
}
\label{fig:nethept}
\caption{Comparisons on NetHept network with Influence Maximization.}
\end{figure}



\begin{figure}[t]
\centering
\subfigure[p2p-Gnutella31]{
\centering
\includegraphics[width=0.22\textwidth]{figures/p2p-time.pdf}
}
\subfigure[NetHept]{
\centering
\includegraphics[width=0.22\textwidth]{figures/nethept-time.pdf}
}
\label{fig:IM-time}
\caption{Comparisons of average oracle evaluations (fixed $\lambda_1$ and $\lambda_2$) on p2p-Gnutella31 and NetHept networks with Influence Maximization.}
\end{figure}




% \pgfplotsset{compat=1.18}

% \begin{figure*}[h]
%     \centering
% \begin{subfigure}[t]{0.245\textwidth}
%   \centering
%   \begin{adjustbox}{width=\linewidth}
%     \begin{tikzpicture}
% \begin{axis}[
% 	xlabel={\Large \textbf{Cost Penalty $\gamma$}},
% 	ylabel={\Large \textbf{Objective ($f-c$)}},
%     legend cell align={left},
%     title={ \Large \textbf{p2p-Gnutella-08 Network}}, legend pos=south west,
%     domain=0:1,cycle list name=mycolorlist1
% ]
% \addplot coordinates{(1.1,4283.47) (1.2,4140.11) (1.3,3959.09) (1.4,3788.44) (1.5,3598.35) (1.6,3450.52) };
% \addplot coordinates{(1.1,3890.59) (1.2,3707.44) (1.3,3472.97) (1.4,3385.57) (1.5,3192.97) (1.6,3025.53) };
% \addplot coordinates{(1.1,4282.33) (1.2,4133.68) (1.3,3946.02) (1.4,3791.52) (1.5,3623.39) (1.6,3431.49) };
% \addplot coordinates{(1.1,4271.85) (1.2,4138.41) (1.3,3943.38) (1.4,3741.19) (1.5,3602.92) (1.6,3412.14) };
% \addplot coordinates{(1.1,4251.61) (1.2,4048.03) (1.3,3850.12) (1.4,3729.32) (1.5,3556.84) (1.6,3336.69) };

% \legend{ROI,UDG,UP$(\epsilon=0.1)$,UP$(\epsilon=0.2)$,UP$(\epsilon=0.5)$}
% \end{axis}
% \end{tikzpicture}
% \end{adjustbox}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.22\textwidth}
%   \centering
%   \begin{adjustbox}{width=\linewidth}
%     \begin{tikzpicture}
% \begin{axis}[
% 	xlabel={\Large \textbf{Cost Penalty $\gamma$}},
% 	% ylabel={Objective ($f-c$)},
%  legend cell align={left},
%     title={ \Large \textbf{NetHept Network}}, legend pos=north east,
%     domain=0:1,cycle list name=mycolorlist1
% ]
% \addplot coordinates{(1.1,10135.4) (1.2,8263.04) (1.3,6842.84) (1.4,5717.57) (1.5,4709.03) (1.6,3990.12) };
% \addplot coordinates{(1.1,8826.89) (1.2,7120.42) (1.3,5784.14) (1.4,4685.47) (1.5,3705.33) (1.6,2917.07) };
% \addplot coordinates{(1.1,10135.5) (1.2,8261.68) (1.3,6845.07) (1.4,5725.41) (1.5,4692.21) (1.6,3996.07) };
% \addplot coordinates{(1.1,10129) (1.2,8266.98) (1.3,6865.59) (1.4,5714.72) (1.5,4686.69) (1.6,3999.01) };
% \addplot coordinates{(1.1,9968.99) (1.2,7890.25) (1.3,6742.73) (1.4,5206.98) (1.5,4599.58) (1.6,3984.47) };

% \legend{ROI,UDG,UP$(\epsilon=0.1)$,UP$(\epsilon=0.2)$,UP$(\epsilon=0.5)$}
% \end{axis}
% \end{tikzpicture}
% \end{adjustbox}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.255\textwidth}
%   \centering
%   \begin{adjustbox}{width=\linewidth}
% \begin{tikzpicture}
%   \begin{semilogyaxis}[
%     ybar,
%     title={\Large \textbf{p2p-Gnutella-08 Network}},
%     symbolic x coords={ROI,  UDG,  UP$(\epsilon=0.1)$, UP$(\epsilon=0.2)$, UP$(\epsilon=0.5)$},
%     bar width=0.5cm, bar shift=-0.3cm,
%     x tick label style={rotate=20, anchor=east},
%     xtick=data,
%     axis y line*=left,
%     ylabel= {\Large \textbf{Function Calls}},
%     % xlabel=(c),
%     ]
%     \addplot[draw=red,fill=red] coordinates {(ROI,87256)
%     (UDG,6082) 
%     (UP$(\epsilon=0.1)$,11037) (UP$(\epsilon=0.2)$,9770) (UP$(\epsilon=0.5)$,8562) 
%     };
%   \end{semilogyaxis}
%   \begin{axis}[
%     ybar,
%     symbolic x coords={ROI,  UDG,  UP$(\epsilon=0.1)$, UP$(\epsilon=0.2)$, UP$(\epsilon=0.5)$},
%     bar width=0.5cm, bar shift=0.3cm,
%     x tick label style={rotate=20, anchor=east},
%     xtick=data,
%     axis y line*=right,
%     ylabel= {\Large \textbf{Time (s)}},
%     ]
%     \addplot[draw=blue,fill=blue] coordinates {
%         (ROI,59.54) 
%     (UDG,19.50) 
%     (UP$(\epsilon=0.1)$,39.55) (UP$(\epsilon=0.2)$,35.66) (UP$(\epsilon=0.5)$,23.08) 
%       };
%   \end{axis}
% \end{tikzpicture}
% \end{adjustbox}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.255\textwidth}
%   \centering
%   \begin{adjustbox}{width=\linewidth}
% \begin{tikzpicture}
%   \begin{semilogyaxis}[
%     ybar,
%     title={\Large \textbf{NetHept Network}},
%     symbolic x coords={ROI,  UDG,  UP$(\epsilon=0.1)$, UP$(\epsilon=0.2)$, UP$(\epsilon=0.5)$},
%     bar width=0.5cm, bar shift=-0.3cm,
%     x tick label style={rotate=20, anchor=east},
%     xtick=data,
%     axis y line*=left,
%     ylabel= {\Large \textbf{Function Calls}},
%     % xlabel=(c),
%     ]
%     \addplot[draw=red,fill=red] coordinates {(ROI,225864) 
%     (UDG,1620) 
%     (UP$(\epsilon=0.1)$,3205) (UP$(\epsilon=0.2)$,3007) (UP$(\epsilon=0.5)$,2423) 
%     };

%   \end{semilogyaxis}
%   \begin{axis}[
%     ybar,
%     symbolic x coords={ROI,  UDG,  UP$(\epsilon=0.1)$, UP$(\epsilon=0.2)$, UP$(\epsilon=0.5)$},
%     bar width=0.5cm, bar shift=0.3cm,
%     x tick label style={rotate=20, anchor=east},
%     xtick=data,
%     axis y line*=right,
%     ylabel= {\Large \textbf{Time (s)}},
%     ]
%     \addplot[draw=blue,fill=blue] coordinates {
%         (ROI,187.61) 
%     (UDG,79.34) 
%     (UP$(\epsilon=0.1)$,119.63) (UP$(\epsilon=0.2)$,109.42) (UP$(\epsilon=0.5)$,87.12) 
%       };
%   \end{axis}
% \end{tikzpicture}

% \end{adjustbox}
% \end{subfigure}


% \caption{Comparisons of unconstrained algorithms on p2p-Gnutella-08 Network and NetHept Network with Profit Maximization Application. The left-side two figures compare the cost penalty $\gamma$ vs. objective $f-c$, and the right-side two charts are for the running time comparisons. We report both the number of function calls (red bars -- corresponds to the left y-axis scale) and actual running time in seconds (blue bars -- corresponds to the right y-axis scale). The function calls are displayed on a logarithmic scale, while the regular y-axis represents the actual running time. The reported time values are the average function calls or actual time of experiments with various cost penalty $\gamma=[1.1,1.2,1.3,1.4,1.5,1.6]$. Similar interpretation applies to Figure \ref{fig:IM-unconstrained-lambda}.} 
%     \label{fig:IM-unconstrained-gamma}
% \end{figure*}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \medskip

% \begin{figure*}[h]
%     \centering
% \begin{subfigure}[t]{0.245\textwidth}
%   \centering
%   \begin{adjustbox}{width=\linewidth}
%     \begin{tikzpicture}
% \begin{axis}[
% 	xlabel={\Large \textbf{Cost Penalty $\lambda$}},
% 	ylabel={\Large \textbf{Objective ($f-c$)}},
%     legend cell align={left},
%     title={ \Large \textbf{p2p-Gnutella-08 Network}}, legend pos=north east,
%     domain=0:1,cycle list name=mycolorlist1
% ]
% \addplot coordinates{(0.1,4134.71) (0.2,3575.4) (0.3,3219.05) (0.4,2963.51) (0.5,2794.29) (0.6,2641.76) };
% \addplot coordinates{(0.1,3715.24) (0.2,3145.58) (0.3,2737.37) (0.4,2622.6) (0.5,2403.24) (0.6,2312.11) };
% \addplot coordinates{(0.1,4131.65) (0.2,3570.49) (0.3,3227.05) (0.4,2976.44) (0.5,2787.93) (0.6,2639.99) };
% \addplot coordinates{(0.1,4120.98) (0.2,3564.32) (0.3,3197.48) (0.4,2954.13) (0.5,2784.68) (0.6,2622.47) };
% \addplot coordinates{(0.1,3985.6) (0.2,3468.24) (0.3,3070.66) (0.4,2856.47) (0.5,2611.5) (0.6,2478.45) };

% \legend{ROI,UDG,UP$(\epsilon=0.1)$,UP$(\epsilon=0.2)$,UP$(\epsilon=0.5)$}
% \end{axis}
% \end{tikzpicture}
% \end{adjustbox}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.22\textwidth}
%   \centering
%   \begin{adjustbox}{width=\linewidth}
%     \begin{tikzpicture}
% \begin{axis}[
% 	xlabel={\Large \textbf{Cost Penalty $\lambda$}},
% 	% ylabel={Objective ($f-c$)},
%  legend cell align={left},
%     title={ \Large \textbf{NetHept Network}}, legend pos=north east,
%     domain=0:1,cycle list name=mycolorlist1
% ]
% \addplot coordinates{(0.1,10890) (0.2,8899) (0.3,7525) (0.4,6312) (0.5,5289) (0.6,4028) };
% \addplot coordinates{(0.1,9468) (0.2,7669) (0.3,6325) (0.4,5306) (0.5,4258) (0.6,3390) };
% \addplot coordinates{(0.1,10885) (0.2,8895) (0.3,7516) (0.4,6301) (0.5,5287) (0.6,4025) };
% \addplot coordinates{(0.1,10701) (0.2,8810) (0.3,7451) (0.4,6268) (0.5,5129) (0.6,3927) };
% \addplot coordinates{(0.1,10480) (0.2,8642) (0.3,7277) (0.4,6037) (0.5,4928) (0.6,3873) };
% \legend{ROI,UDG,UP$(\epsilon=0.1)$,UP$(\epsilon=0.2)$,UP$(\epsilon=0.5)$}
% \end{axis}
% \end{tikzpicture}
% \end{adjustbox}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.255\textwidth}
%   \centering    
%   \begin{adjustbox}{width=\linewidth}
% \begin{tikzpicture}
%   \begin{semilogyaxis}[
%     ybar,
%     title={\Large \textbf{p2p-Gnutella-08 Network}},
%     symbolic x coords={ROI,  UDG,  UP$(\epsilon=0.1)$, UP$(\epsilon=0.2)$, UP$(\epsilon=0.5)$},
%     bar width=0.5cm, bar shift=-0.3cm,
%     x tick label style={rotate=20, anchor=east},
%     xtick=data,
%     axis y line*=left,
%     ylabel= {\Large \textbf{Function Calls}},
%     % xlabel=(c),
%     ]
%     \addplot[draw=red,fill=red] coordinates {(ROI,89681)
%     (UDG,6193) (UP$(\epsilon=0.1)$,9569) (UP$(\epsilon=0.2)$,9420) (UP$(\epsilon=0.5)$,8958) 
%     };  
%   \end{semilogyaxis}
%   \begin{axis}[
%     ybar,
%     symbolic x coords={ROI,  UDG,  UP$(\epsilon=0.1)$, UP$(\epsilon=0.2)$, UP$(\epsilon=0.5)$},
%     bar width=0.5cm, bar shift=0.3cm,
%     x tick label style={rotate=20, anchor=east},
%     xtick=data,
%     axis y line*=right,
%     ylabel= {\Large \textbf{Time (s)}},
%     ]
%     \addplot[draw=blue,fill=blue] coordinates {
%         (ROI,59.94) 
%     (UDG,19.77) 
%     (UP$(\epsilon=0.1)$,38.65) (UP$(\epsilon=0.2)$,35.64) (UP$(\epsilon=0.5)$,22.30) 
%       };
%   \end{axis}
% \end{tikzpicture}

% \end{adjustbox}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.255\textwidth}
%   \centering   
%   \begin{adjustbox}{width=\linewidth}
% \begin{tikzpicture}
%   \begin{semilogyaxis}[
%     ybar,
%     title={\Large \textbf{NetHept Network}},
%     symbolic x coords={ROI,  UDG,  UP$(\epsilon=0.1)$, UP$(\epsilon=0.2)$, UP$(\epsilon=0.5)$},
%     bar width=0.5cm, bar shift=-0.3cm,
%     x tick label style={rotate=20, anchor=east},
%     xtick=data,
%     axis y line*=left,
%     ylabel= {\Large \textbf{Function Calls}},
%     % xlabel=(c),
%     ]
%     \addplot[draw=red,fill=red] coordinates {(ROI,235564) 
% % (LazyROI, 43976)
% (UDG,14121) (UP$(\epsilon=0.1)$,43963) (UP$(\epsilon=0.2)$,37288) (UP$(\epsilon=0.5)$,27547) };
%   \end{semilogyaxis}
%   \begin{axis}[
%     ybar,
%     symbolic x coords={ROI,  UDG,  UP$(\epsilon=0.1)$, UP$(\epsilon=0.2)$, UP$(\epsilon=0.5)$},
%     bar width=0.5cm, bar shift=0.3cm,
%     x tick label style={rotate=20, anchor=east},
%     xtick=data,
%     axis y line*=right,
%     ylabel= {\Large \textbf{Time (s)}},
%     ]
%     \addplot[draw=blue,fill=blue] coordinates {
%         (ROI,187.61) 
%     (UDG,79.33) 
%     (UP$(\epsilon=0.1)$,118.24) (UP$(\epsilon=0.2)$,107.79) (UP$(\epsilon=0.5)$,86.68) 
%       };
%   \end{axis}
% \end{tikzpicture}
% \end{adjustbox}
% \end{subfigure}
% \caption{Comparisons of unconstrained algorithms on p2p-Gnutella-08 Network and NetHept Network with Profit Maximization Application. The left two figures compare the cost penalty $\lambda$ vs objective $f-c$ and the right two charts are for the running time comparisons.}
%     \label{fig:IM-unconstrained-lambda}
% \end{figure*}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[h]
%     \centering
% \begin{subfigure}[t]{0.242\textwidth}
%   \centering
%   \begin{adjustbox}{width=\linewidth}
%     \begin{tikzpicture}
% \begin{axis}[
% 	xlabel={\Large \textbf{number of RR sets ($\times 10^5$)}},
% 	ylabel={\Large \textbf{Objective ($f-c$)}},
%     legend cell align={left},
%     title={ \Large \textbf{p2p-Gnutella-08 Network}}, legend pos=south east,
%     domain=0:1,cycle list name=mycolorlist1,
%     legend columns=2, ymin=2500,
%     xticklabels={$2^1$, $2^2$, $2^3$, $2^4$, $2^5$, $2^6$, $2^7$, $2^8$, $2^9$}, xtick={21,22,23,24,25,26,27,28,29},
% ]
% \addplot coordinates{(21,3674) (22,3797) (23,3878) (24,3947) (25,4005) (26,4068) (27,4114) (28,4157) (29,4177) };
% \addplot coordinates{(21,3412) (22,3488) (23,3542) (24,3590) (25,3624) (26,3654) (27,3676) (28,3685) (29,3694) };
% \addplot coordinates{(21,3665) (22,3777) (23,3868) (24,3928) (25,3986) (26,4055) (27,4102) (28,4134) (29,4168) };
% \addplot coordinates{(21,3642) (22,3756) (23,3846) (24,3921) (25,3968) (26,4036) (27,4085) (28,4114) (29,4154) };
% \addplot coordinates{(21,3621) (22,3733) (23,3800) (24,3877) (25,3921) (26,3985) (27,4036) (28,4066) (29,4088) };

% \legend{ROI,UDG,UP$(\epsilon=0.1)$,UP$(\epsilon=0.2)$,UP$(\epsilon=0.5)$}
% \end{axis}
% \end{tikzpicture}
% \end{adjustbox}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.225\textwidth}
%   \centering
%   \begin{adjustbox}{width=\linewidth}
%     \begin{tikzpicture}
% \begin{axis}[
% 	xlabel={\Large \textbf{number of RR sets ($\times 10^5$)}},
% 	% ylabel={Objective ($f-c$)},
%  legend cell align={left},
%     title={ \Large \textbf{NetHept Network}}, legend pos=south east,
%     domain=0:1,cycle list name=mycolorlist1, legend columns=2, ymin=6500,
%     xticklabels={$2^1$, $2^2$, $2^3$, $2^4$, $2^5$, $2^6$, $2^7$, $2^8$, $2^9$}, xtick={21,22,23,24,25,26,27,28,29},
% ]

% \addplot coordinates{(21,8125) (22,8427) (23,8598) (24,8721) (25,8806) (26,8878) (27,8924) (28,8972) (29,9014) };
% \addplot coordinates{(21,7325) (22,7511) (23,7626) (24,7746) (25,7825) (26,7873) (27,7933) (28,7956) (29,7985) };
% \addplot coordinates{(21,8098) (22,8413) (23,8565) (24,8698) (25,8791) (26,8864) (27,8911) (28,8963) (29,9002) };
% \addplot coordinates{(21,8013) (22,8358) (23,8522) (24,8645) (25,8766) (26,8839) (27,8885) (28,8942) (29,8985) };
% \addplot coordinates{(21,7955) (22,8254) (23,8489) (24,8587) (25,8704) (26,8785) (27,8821) (28,8887) (29,8895) };

% \legend{ROI,UDG,UP$(\epsilon=0.1)$,UP$(\epsilon=0.2)$,UP$(\epsilon=0.5)$}
% \end{axis}
% \end{tikzpicture}
% \end{adjustbox}
% \end{subfigure}
% \caption{Comparisons of unconstrained algorithms on p2p-Gnutella-08 Network and NetHept Network with Profit Maximization Application. These two figures compare the number of RR sets vs objective $f-c$.}
%     \label{fig:IM-unconstrained-rr-obj}
% \end{figure}

% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{figure}[h]
%     \centering
% \begin{subfigure}[t]{0.242\textwidth}
%   \centering
%   \begin{adjustbox}{width=\linewidth}
%     \begin{tikzpicture}
% \begin{axis}[
% 	xlabel={\Large \textbf{number of RR sets ($\times 10^5$)}},
% 	ylabel={\Large \textbf{Time (s)}},
%     legend cell align={left},
%     title={ \Large \textbf{p2p-Gnutella-08 Network}}, legend pos=south east,
%     domain=0:1,cycle list name=mycolorlist1,
%     legend columns=2, ymin=-5,
%     xticklabels={$2^1$, $2^2$, $2^3$, $2^4$, $2^5$, $2^6$, $2^7$, $2^8$, $2^9$}, xtick={21,22,23,24,25,26,27,28,29},
% ]
% \addplot coordinates{(21,52.17) (22,54.24) (23,55.88) (24,57.15) (25,58.35) (26,58.90) (27,59.31) (28,59.54) (29,59.94) };
% \addplot coordinates{(21,13.21) (22,15.44) (23,16.36) (24,17.51) (25,18.27) (26,18.76) (27,19.36) (28,19.50) (29,19.77) };
% \addplot coordinates{(21,32.91) (22,34.42) (23,35.74) (24,36.99) (25,37.89) (26,38.65) (27,39.34) (28,39.55) (29,40.35) };
% \addplot coordinates{(21,30.14) (22,31.55) (23,32.27) (24,33.45) (25,34.69) (26,35.11) (27,35.82) (28,35.66) (29,35.78) };
% \addplot coordinates{(21,15.59) (22,18.56) (23,20.32) (24,21.18) (25,21.98) (26,22.30) (27,22.75) (28,23.08) (29,23.07) };

% \legend{ROI,UDG,UP$(\epsilon=0.1)$,UP$(\epsilon=0.2)$,UP$(\epsilon=0.5)$}
% \end{axis}
% \end{tikzpicture}
% \end{adjustbox}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.225\textwidth}
%   \centering
%   \begin{adjustbox}{width=\linewidth}
%     \begin{tikzpicture}
% \begin{axis}[
% 	xlabel={\Large \textbf{number of RR sets ($\times 10^5$)}},
% 	% ylabel={Objective ($f-c$)},
%  legend cell align={left},
%     title={ \Large \textbf{NetHept Network}}, legend pos=south east,
%     domain=0:1,cycle list name=mycolorlist1, legend columns=2, ymin=0,
%     xticklabels={$2^1$, $2^2$, $2^3$, $2^4$, $2^5$, $2^6$, $2^7$, $2^8$, $2^9$}, xtick={21,22,23,24,25,26,27,28,29},
% ]

% \addplot coordinates{(21,162.25) (22,171.27) (23,177.98) (24,182.21) (25,185.06) (26,186.78) (27,187.61) (28,188.65) (29,188.75) };
% \addplot coordinates{(21,62.25) (22,66.11) (23,70.26) (24,73.46) (25,76.25) (26,78.73) (27,79.33) (28,79.34) (29,79.28) };
% \addplot coordinates{(21,101.98) (22,107.13) (23,111.65) (24,114.95) (25,116.91) (26,118.24) (27,119.11) (28,119.63) (29,120.02) };
% \addplot coordinates{(21,90.16) (22,96.57) (23,100.23) (24,103.44) (25,105.62) (26,107.79) (27,108.66) (28,109.42) (29,109.85) };
% \addplot coordinates{(21,75.55) (22,79.71) (23,82.77) (24,83.96) (25,85.55) (26,86.68) (27,87.21) (28,87.12) (29,87.18) };

% \legend{ROI,UDG,UP$(\epsilon=0.1)$,UP$(\epsilon=0.2)$,UP$(\epsilon=0.5)$}
% \end{axis}
% \end{tikzpicture}
% \end{adjustbox}
% \end{subfigure}
% \caption{Comparisons of unconstrained algorithms on p2p-Gnutella-08 Network and NetHept Network with Profit Maximization Application. These two figures compare the number of RR sets vs Actual Time spent in seconds.}
%     \label{fig:IM-unconstrained-rr-time-s}
% \end{figure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Vertex Cover with Costs}
Let $G=(V, E)$ be a directed graph and $w: 2^V \rightarrow \mathbb{R}^{\geq 0}$ be a modular weight function on a subset of vertices. For a vertex set $S \subseteq$ $V$, let $N(S)$ denote the set of vertices which are pointed to by $S$, formally,
$N(S) \triangleq\{v \in V \mid(u, v) \in E \wedge u \in S\}$. The weighted directed vertex cover function is $f(S)=\sum_{u \in N(S) \cup S} w(u)$, which is monotone submodular. 

We also assume that each vertex $v \in$ $V$ has an associated non-negative cost $c(v)$ \cite{harshaw2019submodular}. We define $c(v)=1+\max \{d(v)-q, 0\}$, where $d(v)$ is the out-degree of vertex $v$ and non-negative integer $q$ is the cost penalty. The minimum cost of a single vertex is $1$. When $q$ is large, the vertex costs are small.

The objective of the {\em vertex cover with costs maximization problem} is to find a subset $S$ such that:

\[\argmax_{S\subseteq V}~ \sum_{u \in N(S) \cup S} w(u) - \sum_{v \in S} c(v)\]

Here, function $f$ is monotone submodular, so we set $\gamma=1$ in Algorithm \ref{alg:up}. 

\medskip

\textbf{Datasets and Experimental Setup}:
We use two networks in the experiment of this application: Protein network \cite{stelzl2005human} and Eu-Email Core network~\cite{leskovec2007graph, yin2017local}. Protein network is a human protein-protein interaction network with $1,706$ nodes (proteins) and $6,207$ edges (interactions). The Eu-Email Core network~\cite{leskovec2007graph, yin2017local}, is a directed graph derived from email data from a European research institution. Comprising 1,005 nodes and 25,571 edges, this graph depicts individuals as nodes and signifies the sending of emails from one individual to another via directed edges, denoted by a directed edge from node $u$ to node $v$. 

Since there is no node weight information in the datasets, for both networks, we assign each node a weight of 1. Additionally, as there is no cost information, we assign costs as mentioned above. For the experiments, we vary cost penalty choices $q \in [1, 12]$ and compare the objective values $(f-c)$ and running time (function calls) of our algorithm UP with ROI, UDG. To see the effect of different error thresholds, we set $\epsilon=0.1, 0.2, 0.5$ for UP. In this application, The function $f$ is submodular ($\gamma=1$), therefore, the distorted marginal profit of the UDG algorithm is $\left(1-\frac{1}{n}\right)^{n-i-1}f(e|S_{i-1})-c(e)$; see the detailed description of the UDG algorithm in Section \ref{sec:related}.

\medskip

\textbf{Results}: Figure~\ref{fig:VC-unconstrained} shows the achieved objective results by each algorithm. When the cost penalty increases, the objective values ($f-c$) also increase for every algorithm. Remarkably, our algorithm demonstrates near-equivalent performance to the best-approximation algorithm \textsc{ROI} with $\epsilon=0.1, 0.2, 0.5$. Even with a larger $\epsilon=0.5$, our algorithm outshines the randomized distorted algorithm \textsc{UDG} by $25\%$ for the Protein network, particularly when dealing with high-cost penalties. The running time comparisons are depicted in the two right-side sub-graphs of Figure~\ref{fig:VC-unconstrained}.
For our algorithms with larger $\epsilon$ values, the running time aligns closely with that of the UDG algorithm, which runs in a clean linear time complexity. In summary, our algorithms demonstrate competitive performance akin to the state-of-the-art while exhibiting comparable linear time execution.


\begin{figure}[t]
\centering
\subfigure[$q$ vs $f-c$; Eu-Email]{
\centering
\includegraphics[width=0.22\textwidth]{figures/email-1.pdf}
}
\subfigure[$q$ vs $f-c$; Protein]{
\centering
\includegraphics[width=0.22\textwidth]{figures/protein-1.pdf}
% \caption{}
}
\label{fig:vertex-cover}
\caption{Comparisons on Eu-Email and Protein networks with Vertex Cover.}
\end{figure}



\begin{figure}[t]
\centering
\subfigure[Vertex Cover]{
\centering
\includegraphics[width=0.22\textwidth]{figures/vertex-cover-time.pdf}
}
\subfigure[Bayesian A-Optimal Design ]{
\centering
\includegraphics[width=0.22\textwidth]{figures/bayesian-time.pdf}
}
\label{fig:VC-bayesian-time}
\caption{Comparisons of average oracle evaluations with Vertex Cover and Bayesian A-Optimal Design.}
\end{figure}




% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \medskip
% \begin{figure*}[h]
%     \centering
% \begin{subfigure}{0.245\textwidth}
%   \centering
%   \begin{adjustbox}{width=\linewidth}
%     \begin{tikzpicture}
% \begin{axis}[ 
% 	xlabel={\Large \textbf{Cost Penalty $q$}},
% 	ylabel={\Large \textbf{Objective ($f-c$)}},
%     title={\Large \textbf{Eu-Email Network}}, legend style={fill=none, nodes={scale=0.8, transform shape}}, legend pos=south east, legend cell align={left},
%     domain=0:1,cycle list name=mycolorlist1
% ]
% \addplot coordinates {(1,75) (2,143) (3,198) (4,235) (5,270) (6,311) (7,353) (8,389) (9,419) (10,448) (11,474) (12,495)};
% \addplot coordinates{(1,36) (2,91) (3,136) (4,162) (5,201) (6,244) (7,298) (8,313) (9,323) (10,373) (11,392) (12,419)};
% \addplot coordinates{(1,75) (2,144) (3,199) (4,237) (5,271) (6,312) (7,354) (8,390) (9,420) (10,449) (11,475) (12,496)};
% \addplot coordinates{(1,77) (2,144) (3,199) (4,237) (5,272) (6,312) (7,352) (8,391) (9,420) (10,450) (11,475) (12,497)};
% \addplot coordinates{(1,68) (2,138) (3,193) (4,227) (5,269) (6,309) (7,346) (8,387) (9,415) (10,443) (11,475) (12,495)};
% % \addplot coordinates{(1,44) (2,28) (3,75) (4,226) (5,256) (6,289) (7,331) (8,329) (9,363) (10,384) (11,417) (12,451) };

% \legend{ROI,UDG,UP$(\epsilon=0.1)$,UP$(\epsilon=0.2)$,UP$(\epsilon=0.5)$}
% \end{axis}
% \end{tikzpicture}
% \end{adjustbox}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.23\textwidth}
%   \centering
%   \begin{adjustbox}{width=\linewidth}
%     \begin{tikzpicture}
% \begin{axis}[
% 	xlabel={\Large \textbf{Cost Penalty $q$}},
% 	% ylabel={Objective ($f-c$)},
%  ylabel near ticks,
%     title={\Large \textbf{Protein Network}}, legend style={fill=none, nodes={scale=1.0, transform shape}}, legend pos=south east,legend cell align={left},
%     domain=0:1,cycle list name=mycolorlist1
% ]

% \addplot coordinates{(1,356) (2,456) (3,528) (4,591) (5,640) (6,683) (7,727) (8,765) (9,809) (10,843) (11,877) (12,911) };
% \addplot coordinates{(1,240) (2,361) (3,425) (4,484) (5,504) (6,540) (7,553) (8,613) (9,642) (10,655) (11,675) (12,703) };
% \addplot coordinates{(1,356) (2,456) (3,528) (4,591) (5,640) (6,683) (7,727) (8,765) (9,808) (10,843) (11,877) (12,911) };
% \addplot coordinates{(1,347) (2,455) (3,534) (4,592) (5,641) (6,683) (7,725) (8,767) (9,810) (10,844) (11,879) (12,913) };
% \addplot coordinates{(1,252) (2,407) (3,475) (4,544) (5,592) (6,648) (7,696) (8,733) (9,780) (10,807) (11,846) (12,892) };

% \legend{ROI,UDG,UP$(\epsilon=0.1)$,UP$(\epsilon=0.2)$,UP$(\epsilon=0.5)$}
%  \end{axis}
% \end{tikzpicture}
% \end{adjustbox}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.245\textwidth}
%   \centering
%   \begin{adjustbox}{width=\linewidth}
% \begin{tikzpicture}  
% \begin{semilogyaxis}  
% [  
%     ybar,  
%     enlargelimits=0.11,  
%     ylabel={\Large \textbf{Function Calls}}, 
%     title={\Large \textbf{Eu-Email Network}},
%     x tick label style={rotate=15, anchor=east},
%     symbolic x coords={ROI, UDG, 
%     UP$(\epsilon=0.1)$, UP$(\epsilon=0.2)$, UP$(\epsilon=0.5)$,} 
%     ]  
% \addplot coordinates {(ROI,225864) 
% % (lazyROI,3859)
% (UDG,1620) 

% (UP$(\epsilon=0.1)$,3205) (UP$(\epsilon=0.2)$,3007) (UP$(\epsilon=0.5)$,2423) 
% };  
% \end{semilogyaxis} 
% \end{tikzpicture} 
% \end{adjustbox}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.23\textwidth}
%   \centering
%   \begin{adjustbox}{width=\linewidth}
% \begin{tikzpicture}  
% \begin{semilogyaxis}  
% [  
%     ybar,  
%     enlargelimits=0.11,  
%     % ylabel={Function Calls}, 
%     ylabel near ticks,
%     title={\Large \textbf{Protein Network}},
%     x tick label style={rotate=15, anchor=east},
%     symbolic x coords={ROI, UDG, UP$(\epsilon=0.1)$, UP$(\epsilon=0.2)$, UP$(\epsilon=0.5)$ 
%     % lazyTROI$(\epsilon=0.75)$
%     }
%     ]  
% \addplot coordinates {(ROI,171961) 
% (UDG,1137) (UP$(\epsilon=0.1)$,2815) (UP$(\epsilon=0.2)$,2638) (UP$(\epsilon=0.5)$,2249)
% % (TROI$(\epsilon=0.75)$,2024)
% };  
% \end{semilogyaxis} 
% \end{tikzpicture} 
% \end{adjustbox}
% \end{subfigure}
% \caption{Comparisons of unconstraint algorithms on Eu-Email and Protein Network with Vertex Cover Application. The left two figures compare the cost penalty $q$ vs objective $f-c$ and the right two charts are for the running time comparisons. The function calls (right-side two sub-plots) are displayed in logarithm scale.}
%     \label{fig:VC-unconstrained}
% \end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure*}[h]
%     \centering

% \begin{subfigure}[t]{0.245\textwidth}
% \begin{adjustbox}{width=\linewidth}
% \begin{tikzpicture}
% \begin{axis}[
% 	xlabel={\Large \textbf{Cost Penalty $p$}},
% 	ylabel={\Large \textbf{Objective Values ($f-c$)}},
%  ylabel near ticks,
%     title={\Large \textbf{Segment Data}}, legend style={fill=white, nodes={scale=1.0, transform shape}},legend cell align={left},
%     legend pos=north east, domain=0:1,cycle list name=mycolorlist1, legend columns=1, ymin=0
% ]
% \addplot coordinates{(0.1,88.2213) (0.2,78.3292) (0.3,69.3882) (0.4,61.4931) (0.5,54.0637) (0.6,48.2272) (0.7,37.551) (0.8,36.0144) (0.9,25.3885) (1,13.9734) };
% \addplot coordinates{(0.1,84.708) (0.2,76.4376) (0.3,67.9481) (0.4,56.6582) (0.5,50.2619) (0.6,42.9344) (0.7,34.2889) (0.8,29.392) (0.9,22.4831) (1,3.55271e-15) };
% \addplot coordinates{(0.1,86.3894) (0.2,77.7228) (0.3,69.4919) (0.4,61.948) (0.5,53.9628) (0.6,47.9004) (0.7,37.8605) (0.8,36.1774) (0.9,23.2792) (1,12.0862) };
% \addplot coordinates{(0.1,86.7952) (0.2,76.1104) (0.3,68.33) (0.4,59.1468) (0.5,51.2405) (0.6,45.3813) (0.7,35.2883) (0.8,35.5426) (0.9,22.2792) (1,12.0862) };
% \addplot coordinates{(0.1,84.4661) (0.2,75.7553) (0.3,66.3387) (0.4,56.5189) (0.5,48.0384) (0.6,43.3812) (0.7,34.5253) (0.8,35.5426) (0.9,21.2792) (1,12.0862) };

% \legend{ROI, UDG, UP$(\epsilon=0.1)$, UP$(\epsilon=0.2)$, UP$(\epsilon=0.5)$}
% \end{axis}
% \end{tikzpicture}
% \end{adjustbox}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.225\textwidth}
% \begin{adjustbox}{width=\linewidth}
% \begin{tikzpicture}
% \begin{axis}[
% 	xlabel={\Large \textbf{Cost Penalty $p$}},
% 	% ylabel={Objective Values},
%  ylabel near ticks,
%     title={\Large \textbf{Housing Data}}, legend style={fill=white, nodes={scale=1.0, transform shape}},legend cell align={left},
%     legend pos=north east, domain=0:1,cycle list name=mycolorlist1, legend columns=1, ymin=0
% ]
% \addplot coordinates{(0.1,75.9589) (0.2,68.0879) (0.3,61.4088) (0.4,54.7298) (0.5,48.0508) (0.6,41.9132) (0.7,36.0466) (0.8,31.0693) (0.9,24.4447) (1,12.3441) };
% \addplot coordinates{(0.1,71.695) (0.2,62.1386) (0.3,52.3771) (0.4,46.9515) (0.5,42.1758) (0.6,35.1654) (0.7,31.9158) (0.8,22.9897) (0.9,15.9539) (1,3.55271e-15) };
% \addplot coordinates{(0.1,74.2249) (0.2,67.3639) (0.3,56.4688) (0.4,49.8476) (0.5,47.6616) (0.6,41.1132) (0.7,35.7124) (0.8,27.0805) (0.9,20.3936) (1,8.52876) };
% \addplot coordinates{(0.1,74.2249) (0.2,67.3639) (0.3,56.4688) (0.4,49.8476) (0.5,46.5595) (0.6,41.1132) (0.7,35.7124) (0.8,26.2218) (0.9,20.3936) (1,8.52876) };
% \addplot coordinates{(0.1,73.4675) (0.2,65.3829) (0.3,55.6876) (0.4,47.4268) (0.5,44.9006) (0.6,38.1132) (0.7,35.7124) (0.8,25.1839) (0.9,19.85013) (1,8.52876) };

% \legend{ROI, UDG, UP$(\epsilon=0.1)$, UP$(\epsilon=0.2)$, UP$(\epsilon=0.5)$}
% \end{axis}
% \end{tikzpicture}
% \end{adjustbox}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.245\textwidth}
%   \centering
% \begin{adjustbox}{width=\linewidth}
% \begin{tikzpicture}  
% \begin{semilogyaxis}  
% [ 
%     ybar,  
%     enlargelimits=0.11,  
%     separate axis lines,
%     ylabel={\Large \textbf{Function Calls}}, ylabel near ticks,
%     title={\Large \textbf{Segment Data}},
%     x tick label style={rotate=15, anchor=east},
%     symbolic x coords={ROI, UDG, UP$(\epsilon=0.1)$, UP$(\epsilon=0.2)$, UP$(\epsilon=0.5)$}, 
%     xtick=data
%     ]  

% \addplot coordinates {
% (ROI,1719614)  
% (UDG,101292) (UP$(\epsilon=0.1)$,484300) (UP$(\epsilon=0.2)$,326356) (UP$(\epsilon=0.5)$,148889)};  
 
% \end{semilogyaxis} 
% \end{tikzpicture} 
% \end{adjustbox}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.225\textwidth}
%   \centering
% \begin{adjustbox}{width=\linewidth}
% \begin{tikzpicture}  
% \begin{semilogyaxis}  
% [  
%     ybar,  
%     enlargelimits=0.11,  
%     % ylabel={Function Calls},
%     ylabel near ticks,
%     title={\Large \textbf{Housing Network}},
%     x tick label style={rotate=15, anchor=east},
%     symbolic x coords={ROI, UDG, UP$(\epsilon=0.1)$, UP$(\epsilon=0.2)$, UP$(\epsilon=0.5)$}, 
%     xtick=data  
%     ]  
% \addplot coordinates {
% (ROI,385643)  
% (UDG,23276) (UP$(\epsilon=0.1)$,277496) (UP$(\epsilon=0.2)$,72314) (UP$(\epsilon=0.5)$,13465)};  
% \end{semilogyaxis} 
% \end{tikzpicture} 
% \end{adjustbox}
% \end{subfigure}
% \caption{Comparisons of unconstrained algorithms on Segment Data and Boston Housing data on Bayesian A-Optimal Design. The left two figures compare the cost penalty $p$ vs objective $f-c$ and the right two charts are for the running time comparisons. The running time measures the total number of function calls using the $\gamma$-GUESS framework.}
%     \label{fig:BAO-unconstrained}
%     % \vspace{-2em}
% \end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Bayesian A-Optimal Design}

Given a measurement matrix $\mathbf{X}=\left[x_1, x_2, \ldots, x_n\right] \in \mathbb{R}^{d}$, a linear model $\boldsymbol{y}_S=\mathbf{X}_S^{\mathrm{T}} \boldsymbol{\theta}+$ $\zeta_S$, a modular cost function $c:2^n \rightarrow \mathbb{R}_{>0}$, where $\boldsymbol{\theta}$ has a Gaussian prior distribution $\boldsymbol{\theta} \sim$ $\mathcal{N}(0, \Sigma)$, the normal i.i.d. noise $\zeta_1, \zeta_2, \cdots, \zeta_n \sim \mathcal{N}\left(0, \sigma^2 \right)$, the objective is to find a submatrix $\mathbf{X}_S$ such that
\[\argmax _{S \subseteq\{1,2, \ldots, n\}} f(S)-c(S)\]

Here 
$f(S)=\operatorname{Tr}(\Sigma)-\operatorname{Tr}\left(\Sigma^{-1}+ \frac{1}{\sigma^{2}} \mathbf{X}_S \mathbf{X}_S^{\mathrm{T}}\right)^{-1}$ is the Bayesian A-Optimality function, which is a non-negative, monotone and $\gamma$-weakly submodular function \cite{bian2017guarantees, harshaw2019submodular}. $\operatorname{Tr}(\cdot)$ denotes the trace of a matrix. 

Moreover, the marginal gain of adding a measurement $e$ to $S$ can be efficiently calculated by:

\[f(e | S)=\frac{||z_e||^2}{\sigma^2+\left\langle x_e, z_e\right\rangle}\]

where $z_e=\mathbf{M}_S^{-1} x_e$ and $\mathbf{M}_S=\Sigma^{-1}+\mathbf{X}_S \mathbf{X}_S^T$

The cost of a measurement $e \in [n]$ is defined to be proportional to its $f$ value. The modular cost of set $S$ is $c(S)=\sum_{e \in S} c(e) = p\sum_{e \in S}f(e)$, where $p$ is the cost penalty.

\begin{algorithm}[tb]
   \caption{\textsc{$\gamma$-guess}($f, c, \delta, \epsilon$)}
    \label{alg:guess}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} utility function $f$, cost function $c$, decay threshold $\delta$, error threshold $\epsilon$ for Algorithm UP
   \STATE {\bfseries Output:} $S = \argmax_{S_r, r\leq T}\{ f(S_r)-c(S_r) \}$
   \vspace{.05in}
     \STATE  $T \gets \Big\lceil \frac{1}{\delta}\ln \frac{1}{\delta} \Big\rceil$
    \STATE $S_0 \gets \emptyset$
    \FOR{$r \gets 0 ~to~ T$}
      \STATE  $\gamma_r \gets (1-\delta)^r$
      \STATE  $S_r \gets \textsc{UP}(f,c,\gamma_r,\epsilon)$ or $ \textsc{UDG}(f,c,\gamma_r)$
      \STATE  $r++$
    \ENDFOR
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \Input{utility function $f$, cost function $c$, decay threshold $\delta$, error threshold $\epsilon$ for Algorithm UP}
%     \Output{$S = \argmax_{S_r, r\leq T}\{ f(S_r)-c(S_r) \}$}
%     $T \gets \Big\lceil \frac{1}{\delta}\ln \frac{1}{\delta} \Big\rceil$\\
%     $S_0 \gets \emptyset$\\
%     \For{$r \gets 0 ~to~ T$}{
%         \tcc{geometrically decay the submodularity ratio from 1}
%         $\gamma_r \gets (1-\delta)^r$\\
%         \tcc{get a solution set from an algorithm taking $\gamma_r$, depending on the running algorithms}
%         $S_r \gets \textsc{UP}(f,c,\gamma_r,\epsilon)$ or $ \textsc{UDG}(f,c,\gamma_r)$\\
%         \smallskip
%         $r++$
%     }
%     \caption{\textsc{$\gamma$-guess}($f, c, \delta, \epsilon$)}
%     \label{alg:guess}
% \end{algorithm}

\medskip

\textbf{Datasets and Experimental Setup:} 
We use the Boston Housing dataset \cite{harrison1978hedonic}, Segment Data\footnote{https://www.csie.ntu.edu.tw/$\sim$ cjlin/libsvmtools/datasets/multiclass.html\#segment} that was used in \cite{qian2021multiobjective}. 
The Boston Housing dataset is a typical benchmark dataset encompassing $d = 14$ attributes detailing information about $n = 506$ Boston houses. These attributes cover various factors such as the average number of rooms per dwelling, proximity to the Charles River, and the crime rate per capita. The Segment data has $n=2,310$ entries and $d=19$ features. To prepare the datasets for analysis, we performed pre-processing tasks that involved normalizing the features to achieve a zero mean and a standard deviation of 1.
In the Bayesian A-Optimality function $f(S)$, we set $\sigma=1/\sqrt{d}$.

In the experiment on Bayesian A-Optimal Design, as the submodularity ratio is not known apriori, we implemented a standard
algorithm $\gamma$-\textsc{Guess} to \emph{estimate} an approximate $\gamma$. We follow the submodularity ratio guessing algorithm in~\cite{harshaw2019submodular}, as per Algorithm \ref{alg:guess}. The algorithm executes Algorithm $\textsc{UP}$ or UDG for a total of $T=\lceil \frac{1}{\delta}\ln \frac{1}{\delta} \rceil$ iterations. At each iteration $r$, there is a distinct submodularity ratio $\gamma_r$. The algorithm takes this $\gamma_r$ for the solution set selection in Line 4. The outputs of Algorithm \ref{alg:guess} is the set with the maximum objective value and the total number of function call.
For the UWSM problem, we fix the decay threshold $\delta=0.2$ in Algorithm \ref{alg:guess}. We compare the objective values $(f-c)$ and running time (number of function calls) with various cost penalty choices $p=[0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1.0]$. For our algorithm UP, we also test various error thresholds $\epsilon=0.1, 0.2$, and $0.5$.

\smallskip

\textbf{Results}: For Bayesian A-Optimality, the objective $f-c$ and running time comparisons are plotted in Figure~\ref{fig:BAO-unconstrained}. 
The quality of the result obtained from ROI (as a heuristic) is validated against other algorithms (including ours) with specific approximation guarantees, but it needs the highest number of function queries. As for the objective values, the density maximization-based algorithms (ROI and UP) produce higher-quality solutions than UDG.  As for running time, compared to the linear-time baseline UDG, our algorithm UP with high error threshold $\epsilon=0.5$ runs faster. A possible explanation  is that our algorithm in Line 6 removes all possible elements that will cause the objectives to decrease. In contrast, UDG will sample an element for exactly $n$ times and evaluate the marginal profit every time. 


\begin{figure}[t]
\centering
\subfigure[$p$ vs $f-c$; Segment]{
\centering
\includegraphics[width=0.22\textwidth]{figures/segment-1.pdf}
}
\subfigure[$p$ vs $f-c$; Housing]{
\centering
\includegraphics[width=0.22\textwidth]{figures/housing-1.pdf}
% \caption{}
}
\label{fig:bayesian}
\caption{Comparisons on Segment and Boston Housing data with  Bayesian A-Optimal Design.}
\end{figure}
